MUSE: Textual Attributes Guided Portrait Painting Generation

We propose a novel approach, MUSE, to illustrate textual attributes visually via portrait generation. MUSE takes a set of attributes written in text, in addition to facial features extracted from a photo of the subject as input. We propose 11 attribute types to represent inspirations from a subject's profile, emotion, story, and environment. We propose a novel stacked neural network architecture by extending an image-to-image generative model to accept textual attributes. Experiments show that our approach significantly outperforms several state-of-the-art methods without using textual attributes, with Inception Score score increased by 6% and Fr\'echet Inception Distance (FID) score decreased by 11%, respectively. We also propose a new attribute reconstruction metric to evaluate whether the generated portraits preserve the subject's attributes. Experiments show that our approach can accurately illustrate 78% textual attributes, which also help MUSE capture the subject in a more creative and expressive way.

==> 3.4analysis.tex <==


\subsection{Qualitative Analysis}


% \heng{need to list many pairs to show the difference between baseline and MUSE output}
% \heng{artist style modeling. need to some clustering of the existing paintings of the artist. }
% %\heng{portrait to portrait?}

% \heng{show style transfer results, using the same photo as input, and change the input text attributes to show different results when the text attribute changed from young to old, from man to woman}

% \heng{show how portraits change over epochs}




%%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%%%%%%%%
% Test Phase:
% Input: a subject's photo or old painting, text description, structured attributes, the artist's old paintings
% Output: a new painting about the new subject
% But we don't have many training pairs of <photo, painting>, so we have tried to cluster all portrait paintings from WikiData according to the artisits, some statistics below.
% Here are the links to visualized portraits along with their text descriptions and attributes:
% XXX
% Pengfei
% =======================
% 7086, anonymous
% 1330, [NULL]
% 463, Rembrandt
% 330, Boris Chaliapin
% 251, Anthony van Dyck
% 250, Nicolaes Maes
% 248, Frans Hals
% 218, George Dawe
% 193, Pierre-Auguste Renoir
% 190, Peter Lely
% 179, Vincent van Gogh
% 164, Eliseu Visconti
% 159, Francisco Goya
% 154, Bartholomeus van der Helst
% 141, Corneille de Lyon
% 138, Peter Paul Rubens
% 134, Pablo Picasso
% 133, Jacek Malczewski
% 132, Kees Verwey
% 128, Titian
% 124, Amedeo Modigliani
% 118, Michiel van Mierevelt
% 118, Gilbert Stuart
% 116, Gerard ter Borch
% 113, Joshua Reynolds
% 112, Joshua Johnson
% 103, Paul Cézanne
% 102, Godfrey Kneller
% 101, Jan van Ravesteyn
% 101, Caspar Netscher


==> backup/3.3results.tex <==
\subsection{Generation of Attributes}


\heng{to save space you can remove the final two rows of figure 6; 
and remove the bottom part of figure 7's the first column (results not good), the fifth column (people may think it as data bias racism)
the sixth column (results not good)}


% \heng{add price results}


% \heng{overall results}
% \heng{add comparison with a baseline without text attribute input}

% \heng{when artist is the same:}
% % We are generating a new painting based on the old paintings from the same artist.

% \heng{put up a subject confusion matrix here}
We check if generated portraits reflect the input attribute values, and further explore how attribute semantics are learned and grounded into generated portraits.

% \bo{we need to mention what metrics we use to define coherence here}

\noindent\textbf{Subject Attribute Reconstruction Accuracy.} Since most of ImageNet classes are objects and the number of classes that appear in portraits is quite limited, the IS metric cannot evaluate the subtle details of human subjects in portraits. 
%We propose the following two new \emph{Subject Reconstruction} metrics designed for portraits. 
Thus we ask \emph{What’s That All About?} by looking for entity attributes, and \emph{How’d They Do That?} by checking the style of the portrait. We ask a human assessor to tag entity attributes on each generated portrait, and compute the F-score of the tagged attributes against the attributes extracted from the text description. 
\heng{where is attribute reconstruction metric? recover it here}

\noindent\textbf{Single Attribute Coherence} We first consider a simpler scenario where we consider changing only one attribute. We train separate models for each attribute, for which we constrained the attribute embeddings $\mathbf{v}$ to contain only the specific attribute (e.g. \texttt{hair}) during training. 

Figures \ref{fig:hair},\ref{fig:face},\ref{fig:gender} show example outputs modifying \texttt{hair}, \texttt{face expression} and \texttt{gender} respectively. 
% show different style transfer results, which use the same photo as input and only change one of input text attributes. 
We can see models are mostly successful in changing these attributes. We also show results of baseline model here, which take no attribute information as input during both training and testing phase. Therefore, baseline outputs reflect the distribution of training data. For example in Figure~\ref{fig:hair}, we notice baseline outputs always tend to have close-to-brown hairs regardless of input photos due to training data bias. Therefore, success in generating \texttt{blond} and \texttt{black} hair demonstrates that \Model{} is indeed learning to generate according to attribute values rather than some random behavior.

We also notice the varying difficulty of learning different attributes. Results on \texttt{face expression} in Figure \ref{fig:face} are not equally successful as \texttt{hair}, especially for some less frequent values such as \texttt{quizzical expression} for which only generated portraits on second and last row looks indeed ``quizzical''. Besides we find that although it is usually hard to convert an smiling photo into completely \texttt{blank expression}, they usually looks less happier than generated portraits with \texttt{smile} faces.

In addition, we present results on \texttt{gender} attribute because it is a more abstract concept compared with the \texttt{hair} or \texttt{face expression} and cannot be directly grounded into specific facial features. Note that our purpose is not to judge gender based on facial appearance, but rather examine if the generator can learn some common features among various groups by the time these portraits were created. We show \texttt{male} and \texttt{female} results, for which we have enough data for training and evaluation. It is shown in Figure \ref{fig:gender} that \Model{} can automatically learn some low level features to ground the abstract attribute, such as redder mouths in \texttt{female} portraits and more beards in the \texttt{male} portraits.
% , given an input photo, different portraits are generated by using different hair attribute values `Blond Hair', `Black Hair', `Wavy Hair', `Straight Hair' and `Short Hair', respectively. 
% For example, the subject of the input photo in the first row is a lady with black hair. With the input attribute value `Blond Hair', the hair of the subject in the generated portrait has changed to blond. Similarly, the subject of the input photo in the fourth row has a long hair. With the input `Short Hair', the hair of the subject of the generated portrait is relatively shorter than that of the input photo. In Figure \ref{fig:face}, the subjects of generated portraits with `smile' attribute value have a mouth lifted upper and deeper wrinkle than that generated with `Blank Expression'. In Figure \ref{fig:gender}, the generated portrait with `Female' attribute value has a redder mouth while the generated portrait with `Male' attribute value has more beards.

\noindent\textbf{Multiple Attributes}
Figure \ref{fig:combined} shows the system generated portraits at different epochs using a combination of 11 attributes listed in Table \ref{tab:dimensions}. With a mixture of attributes, \emph{\Model{}} can simultaneously generate a portrait that matches most of the attributes. For example, the first column shows the generated portraits from the baseline and the \emph{\Model{}}. As we can see, the generated portrait from the baseline model is visually similar to the input photo with unexpected changes in color and lights. Unlike the baseline model, the portrait generated by \emph{\Model{}} not only has a visual portrait style, the subject in the portrait is a young female with a calm mood and a black hair, which is consistent with the input attributes.



% A quantitative comparison between the baseline and the proposed \emph{\Model{}} using IS and FID performance metrics is shown in Table \ref{tab:IS&FID}.
% The qualitative comparison between the baseline method and the proposed \emph{\Model{}} by inputting a single attribute or a combination of multiple attributes, respectively, is shown in Figure \ref{fig:hair},\ref{fig:face},\ref{fig:gender},\ref{fig:combined}.



\noindent\textbf{Grounding of Attributes}
We further examine how the model ground attributes into generated portraits, by taking an demonstrative example of the \texttt{hair} attribute as shown in Figure \ref{fig:grounding}. 
% we evaluate our model's ability of visual grounding of abstract concepts with small data. 
Five fake faces are designed for the \texttt{hair} attribute and taken as input photo to the \Model{}. In the first two columns are blank face outlines with no/simplified facial features. In the third column \Model{} is presented with only facial features, without outline of the face. From these results we observe that \Model{} can rely on either face outlines or facial features such as eyes or mouths to estimate the relative position of components including hair and facial area. In the fourth column we design a blank face with hair outline. Although \Model{} cannot perfectly color the hair area, we do observe it tend to color along the lines. We also show in the last column that \Model{} works in the similar way for faces in profile.
\begin{figure}[t]
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccc}
\rotatebox[origin=c]{90}{\small{Input Photo}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00214A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00210A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00209A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00211A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00216A_001.jpg}} & \\
\rotatebox[origin=c]{90}{\small{Blond Hair}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00214_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00210_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00209_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00211_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00216_blond.png}} \\
\rotatebox[origin=c]{90}{\small{Black Hair}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00214_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00210_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00209_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00211_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/ground/00216_black.png}} \\
\end{tabular}}
\caption{Given drawn sketches and an attribute of hair color or weather, the attribute value can be correctly grounded in the generated portraits.}
\label{fig:grounding}
\end{figure}

\noindent\textbf{Inter-dependency of Attributes}
As discussed in \ref{sec:EntityTyping}, the attribute values in Table \ref{tab:dimensions} are correlated. Here we pick the weather and mood attributes as an example to evaluate their dependency. As can be seen in Figure \ref{fig:dependency}, by changing the weather attribute value from `rainy' to `sunny', the subject mood inferred from the generated portraits is also changed from `sad' to `happy'.

\begin{figure}[t]
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccc} 
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00011A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00011_stormy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00011_sad.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00011_sunny.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00011_happy.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00024A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00024_stormy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00024_sad.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00024_sunny.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00024_happy.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00150A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00150_stormy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00150_sad.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00150_sunny.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00150_happy.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00189A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00189_stormy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00189_sad.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00189_sunny.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/depend/00189_happy.png}} \\
Input Photo & Stormy & Sad & Sunny & Happy \\
\end{tabular}}
\caption{Inter-dependency of attributes.}
\label{fig:dependency}
\end{figure}



\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccccc} \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_wavy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_straight.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00005_short.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_wavy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_straight.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00042_short.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_wavy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_straight.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00095_short.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_wavy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_straight.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00148_short.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_blond.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_black.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_wavy.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_straight.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/hair/00158_short.png}} \\
Input Photo & \parbox{1.8cm}{\centering Human Generated} & Baseline & Blond Hair & Black Hair & Wavy Hair & Straight Hair & Short Hair \\
\end{tabular}
\caption{Synthetic portraits of the proposed \emph{\Model{}} trained on our portrait dataset given an attribute of hair color.}
\label{fig:hair}
\end{figure*}


\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccccc} \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_smile.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_blank.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_glance.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_quizzical.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00014_smirk.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_smile.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_blank.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_glance.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_quizzical.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00021_smirk.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_smile.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_blank.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_glance.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_quizzical.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00090_smirk.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_smile.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_blank.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_glance.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_quizzical.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00124_smirk.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_smile.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_blank.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_glance.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_quizzical.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/face/00187_smirk.png}} \\
Input Photo & \parbox{1.8cm}{\centering Human Generated} & Baseline & Smile & \parbox{1.8cm}{\centering Blank Expression} & Glance & \parbox{1.8cm}{\centering Quizzical Expression} & Smirk \\
\end{tabular}
\caption{Synthetic portraits of the proposed \emph{\Model{}} trained on our portrait dataset given an attribute of face expression.}
\label{fig:face}
\end{figure*}




\begin{figure}[t]
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccc}
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00056A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00056.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00056_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00056_female.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00056_male.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00134A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00134.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00134_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00134_female.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00134_male.png}} \\
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00151A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00151.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00151_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00151_female.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00151_male.png}} \\
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00171A_001.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00171.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00171_base.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00171_female.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00171_male.png}} \\
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00198A_001.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00198.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00198_base.png}}
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00198_female.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/gender/00198_male.png}} \\
Input Photo & \parbox{1.8cm}{\centering Human Generated} & Baseline & Female & Male \\
\end{tabular}}
\caption{Synthetic portraits of the proposed \emph{\Model{}} trained on our portrait dataset given an attribute of gender. \bo{maybe add MUSE in the method names, o/w it's not quite clear which columns are generated by the proposed method}}
\label{fig:gender}
\end{figure}



\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccccccc}
\rotatebox[origin=c]{90}{\small{Input Photo}} & \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00089A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00022A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00024A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00026A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00053A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00054A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00060A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00074A_001.jpg}} \\
\rotatebox[origin=c]{90}{\scriptsize{Human Generated}} & \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00089.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00022.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00024.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00026.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00053.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00054.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00060.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00074.jpg}} \\
\rotatebox[origin=c]{90}{\small{Baseline}} & \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00089_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00022_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00024_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00026_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00053_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00054_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00060_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00074_base.png}} \\
\rotatebox[origin=c]{90}{\scriptsize{System Generated}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00089_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00022_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00024_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00026_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00053_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00054_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00060_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00074_epoch1000.png}} \\
& \scriptsize{\parbox{1.8cm}{\centering Classical Art; Sitting; Stormy; Foggy; Blank Expression; Black hair}} & \scriptsize{\parbox{1.8cm}{\centering Calm; Classical Art; Sitting; Rainy; Cold; Male; Black hair; Short hair}} & \scriptsize{\parbox{1.8cm}{\centering Calm; Modernism; Standing; Sunny; Dress; Straight hair}} & \scriptsize{\parbox{1.8cm}{\centering Young adults; Impressionism; Sitting; Cloudy; Long Face; Female; Hat; Black hair}} & \scriptsize{\parbox{1.8cm}{\centering Young adults; Calm; Classical Art; Before 1970; Stormy; Frown; Glance; Male; Coat; Blond hair}} & \scriptsize{\parbox{1.8cm}{\centering Young adults; Impressionism; Standing; In the room; Female; Hat; Blond hair}} & \scriptsize{\parbox{1.8cm}{\centering Young adults; Calm; Classical Art; Sitting; Sunny; Smile; Female; Dress; Wavy hair; Blond hair}} & \scriptsize{\parbox{1.8cm}{\centering Calm; Impressionism; Sitting; Stormy; Cloudy; Female; Dress; Black hair}}
\\
\rotatebox[origin=c]{90}{\small{Input Photo}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00075A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00088A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00006A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00090A_001.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00092A_001.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00093A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00154A_001.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00191A_001.jpg}} \\
\rotatebox[origin=c]{90}{\scriptsize{Human Generated}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00075.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00088.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00006.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00090.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00092.jpg}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00093.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00154.jpg}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00191.jpg}} \\
\rotatebox[origin=c]{90}{\small{Baseline}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00075_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00088_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00006_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00090_base.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00092_base.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00093_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00154_base.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00191_base.png}} \\
\rotatebox[origin=c]{90}{\scriptsize{System Generated}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00075_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00088_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00006_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00090_epoch1000.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00092_epoch1000.png}} &
% \ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00093_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00154_epoch1000.png}} &
\ctab{\includegraphics[height=1.8cm,keepaspectratio]{wacv2021/figure/results2/combined/00191_epoch1000.png}} \\
& 
% \scriptsize{\parbox{1.8cm}{\centering Child; Happy; Classical Art; Sitting; Hot; Female; Blond hair}} &
\scriptsize{\parbox{1.8cm}{\centering Calm; Classical Art; Modernism; Sitting; Stormy; Hat; Black hair}} &
\scriptsize{\parbox{1.8cm}{\centering Calm; Impressionism; Sitting; In the room; Sunny; Female; Dress; Wavy hair}} & 
\scriptsize{\parbox{1.8cm}{\centering Calm; Standing; In the courtyyard or a garden; Sunny; Female; Dress; Straight hair; Blond hair}} &
% \scriptsize{\parbox{1.8cm}{\centering Realism; Sitting; In the room; Sunny; Smile; Female; Dress; Hat}} &
% \scriptsize{\parbox{1.8cm}{\centering Young adults; Calm; Classical Art; Before 1970; In the room; Sunny; Female; Dress; Straight hair}} & 
\scriptsize{\parbox{1.8cm}{\centering Happy; Classical Art; Sitting; Sunny; Smile; Female; Dress; Wavy hair}} &
\scriptsize{\parbox{1.8cm}{\centering Calm; Classical Art; Sitting; Cold; Blank Expression; Female; Dress; Wavy hair; Black hair}}
\end{tabular}
\caption{Synthetic portraits of the proposed \emph{\Model{}} trained on our portrait dataset givin combined attributes including age, mood, style, time, pose, setting, weather, face expression, gender, clothing and hair.}
\label{fig:combined}
\end{figure*}



==> backup/attention.tex <==
\subsection{Inter-modal Attention Model}
\label{sec:Inter-modal}
The model contains $N$ image generation networks $(G_0, G_1, ..., G_{N-1})$ stacked sequentially. Let $\mathbf{m}$ denote a concatenation of the image features $\mathbf{\tilde{x}}$ (Section \ref{sec:ImageEncoder}), the text features $\mathbf{c}$ (Section \ref{sec:textAttn}) and the noise vector $\mathbf{z}$ as the input features to inform the multi-stage image generation model about the content of photo $x$ and text descriptions $t$. Let $h_0$ represent the hidden image features of $m$.

In this step we leverage inter-modal attention~\cite{AttnGAN}, denoted as $F_i^{\textit{attn}}, (i=0,1,...,N)$, to map the text features into a text-image common semantic space in order to generate images most relevant to the input words and entity attributes.
At the $i^{\textit{th}}$ stage, the input image features $\mathbf{h}_i$ are the output from the last stage. %\heng{very unclear and ambiguous about 'stage', can you elaborate and re-phrase}
Next, the text features $\mathbf{c}$ extracted from the text encoder (Section \ref{sec:textAttn}) are transformed into the text-image semantic space as $q(\mathbf{c})=\mathbf{W}_{q} \mathbf{c}$, where $\mathbf{W}_{q}$ is a learnable weight matrix. 

Then, a normalized factor $\beta_{i,j,n}$, which indicates the similarity between the $n^{th}$ attribute and the $j^{th}$ image region, is computed as:
\begin{equation}
\beta_{i,j,n} = \frac{\exp{(s'_{i,j,n})}}{\sum_{\hat{n}=1}^{N_i^w}\exp{(s'_{i,j,\hat{n}})}}
\label{eq:beta}
\end{equation}
where $N_i^w$ is the number of attributes and $s'_{i,j,n} = \mathbf{h}_{i,j}^{\top} q(\mathbf{c}_n)$. Then, a attribute-context vector $p_{i,j}$ corresponding to the $j^{th}$ region of $\mathbf{h}_i$ is obtained by weighting the attribute features $q(\mathbf{c}_n)$ with the normalized factor $\beta_{i,j,n}$ as
\begin{equation}
\mathbf{p}_{i,j} = {\textstyle\sum_{n=1}^{N_i^w}} \beta_{i,j,n}q(\mathbf{c}_n)
\label{eq:word_context}
\end{equation}
Finally, the attribute-context vectors $\mathbf{p}_i$ and image features $\mathbf{h}_i$ are stacked together to be fed into the next stage of the proposed MUSE network architecture.


==> backup/bak.tex <==
%Contributions:
%1. the first portrait generation task that leverages text description
%2. new data augmentation method: use portrait to generate photo to expand training data
%3. method: LSTM only for text -> we apply fine-grained entity extraction to extract attributes for subject and artist, and environment
%attention-GAN; object detection? 
%emotion detection from image and text? happy -> smiling face?
%use bootstrapping to augment text descriptions
%4. new data set and benchmark
% add dimensions from email 


% we ask if we feed an AI enough existing pairs of painting text descriptions, will it learn the artist's style and the subject's life, can we incrementally generate new portrait from old portraits? if we change the subject, can we generate?
% In this paper, we 

% artist style modeling. need to some clustering of the existing paintings of the artist. 

% clothing details. black tie
%portrait is a special type of painting... because of 
% most portraits have a prototype.... muse; give examples; inspiration
% multimedia input; mood etc. 



%%%%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%%%%%%%%
%' ; the implicit attributes of the subject are provided for style control, the model should generate a portraint...generate given a text describing
%1. portrait generation is not just about visual features, we need to look at subject, environment, etc. so we need to incorporate text descriptions and text attributes
%we need content (photo+text) and style control (text)
%text description may come from environment and from subject and artist

%2. challenges: no input photo for most portraits because they are from long time ago -> data augmentation: why imperfect photos can be used for training? existing portrait-photo generator can capture some basic visual feature transfer
%evaluate....automatic metric only look at decipher attributes...tag emotions...
%missing elements...what's in a portrait?

%evaluation: walk into museum, appreciation not just from color visual, but more about the story behind it striking
%choose a set of attributes, tag each system generated portrait, F-score.


==> backup/overview.tex <==
% \subsection{Overview}
\label{sec:Architecture}


% The system outputs a portrait given the facical features from input photo and attributes in text form as input. 
% The facial features of the input photo are extracted by face parsing. %, and the attributes are encoded. 
% Then both the facial features and the text attribute features are stacked together and projected into a multimedia common semantic space. The portrait generation networks take the vectors from the multimedia common semantic space to generate the facial components with the style consistent with the input attributes. Finally, the portrait is generated by blending the generated pixels of the eye, lip and skin regions using Poisson blending. %\heng{revise caption to make it more concrete} 
%\heng{Attributes Encoder -> Attribute Encoder}
\begin{figure*}[!ht]
\centering
\begin{tabular}{c}
\includegraphics[width=16cm,keepaspectratio]{coling2020/img/Networks5.png}
\end{tabular}
\caption{Overview of the generation networks. Given the text context vector $c$ and 
\bo{need to explain the notations a bit here, what is c, m? }}
\label{fig:overview2}
\end{figure*}
% \heng{this overview summarizes what you did, but not why you did in this way, what are the advantages and motivations, elaborate that at the beginning and in the middle of detailed descriptions}
% \heng{in addition to entity attributes, i think we should keep the original text as input
% similar to https://www.ccs.neu.edu/home/luwang/papers/EMNLP2019\_sharma\_huang\_hu\_wang.pdf
% maybe both entity attribute attention and text description attention}
% \heng{put in overall figure here, the figure should include a multimedia common semantic space that combines entity attributes, words, and images}
% \heng{so the overall design is: we obtain some text representation from unstructured text description and structured text attributes, and visual representation from the image photo, then combine them through cross-modal attention. need to write this more clearly and elaborate motivation.}
% The system outputs a portrait given the facical features from input photo and attributes in text form as input, which is expected to match the subject of photo and content/style information specified by attributes.
% given an input photo and text description of the target portrait, the task is to generate a portrait with virtual features matching the content and style information inferred from the photo and text description, respectively. 




% We apply a self-attention-based image encoder \cite{SAGAN} to extract visual features $\mathbf{x}$ from the facial features $x$.
% which captures non-local inter-dependencies among spatially separated image regions. 

%From an input text description $t$, we apply an open-domain fine-grained entity discovery and linking system \cite{Ying2019attentive} to extract entities $e$ and their attributes $a$ \heng{fine-grained entity extraction can only give you entities, not attributes, revise this paragraph to accurately describe how you obtain attributes}. 
% To allow the model to focus on more informative words in the input attributes written in text, we represent an entity context vector $c^e$ 
%and a sentence context vector $c^r$
% with attention mechanisms (Section \ref{sec:textAttn}) \heng{this needs to be fixed, since we don't have sentence any more}. Both the entity context vector $c^e$ and the sentence context vector $c^r$ are then concatenated as an input to \emph{MUSE}, denoted as $c$.


% Since the latent space for the entity embedding is usually high dimensional,  with limited amount of data, it usually causes discontinuity in the latent data manifold. In order to obtain more training pairs given a small number of image-text pairs, an conditioning augmentation technique \cite{ZhangXLZHWM16}, denoted as $F^{\textit{ca}}$, is applied, which randomly samples the latent variables $\hat{e}$ from an independent Gaussian distribution $\mathcal{N} (\mu(\tilde{e}),\Sigma(\tilde{e}))$ where the mean $\mu(\tilde{e})$ and diagonal covariance matrix $\Sigma(\tilde{e})$ are functions of the entity
% embedding $\tilde{e}$. The augmented entity
% embeddings $\hat{e}$ stacked with the input photo features $\tilde{x}$ and a noise vector $z \sim \mathcal{N}(0,1)$ allowing for considerable flexibility in generation \cite{MirzaO14} to construct the input to the generative network, which consists of three stages connected in cascade. \Xiaodan{Conditioning augmentation may be unnecessary.}


The generation model contains $N$ image generation networks $(G_0, G_1, ..., G_{N-1})$ and $N$ corresponding discriminator networks $(D_0, D_1, ..., D_{N-1})$ stacked sequentially for simultaneous adversarial training.
At the beginning of the first stage, the encoded facial features $x$, encoded text features $c$ are concatenated to form the conditional input to the generation networks. The final input to generatio networks is $m=[\mathbf{x};\mathbf{c};\mathbf{z}]$, where $\mathbf{z}$ is the standard Gaussian noise to model the randomness.
% \heng{what is noise vector? why do we need to add it? explain} are concatenated as $m$ in the multimedia common semantic space. 
Let $h_0$ represent the hidden image features of $m$. At the first stage, the generator $G_0$ takes the image features $h_0$ to generate portrait $\hat{x}_0$ and the discriminator $D_0$ takes the generated portrait $\hat{x}_0$ together with corresponding golden portrait $y_0$ to evaluate the generator $G_0$. At the same time, attribute-context vectors $\hat{c}$ are obtained by transforming the text features $c$ into the text-image semantic space (Section \ref{sec:Inter-modal}). Both the attribute-context vectors $\hat{c}$ and the image features $h_0$ are stacked together to be fed into the second stage. In recursion, the generator $G_{N-1}$ at the last stage generates the portrait $\hat{x}_{N-1}$.

% Each generator $G_i$ has a corresponding discriminator classifier $D_i$ to classify the $i^{th}$ synthesized image into a real or false class. The generator $G_i$ expands the noise samples $z$ to the synthetic
% portrait images while the discriminator evaluates the generator. The better the generator, the more likely that the discriminator will be fooled. At the same
% time, the discriminator is being trained to increase its ability to distinguish false from real content by minimizing the loss between the output score and the ground truth. Moreover, at each stage, \emph{MUSE} uses transposed convolution to facilitate the learning efficiency. 

At the final stage, we apply an image encoder based on a convolutional neural network architecture to compute an image-text matching score between the synthesized image and its text description.

Each $G_i$ and $D_i$ is constructed alternately by using a set of image and text-image loss functions (as shown in Figure \ref{fig:overview2} and Section \ref{sec:LossFunction}) solved by gradient descent, where $G_i$ and $D_i$ are consisting of one convolutional layer and four to eight convolutional layers, respectively.

The details of each component are described in the following subsections.

\heng{in the next subsections you need to walk the formulas through the example}

\bo{as an overview section, it is a bit long. I think a better structure is: 1. in fig 2, you add name for each block in the figure, such as image encoder, text extractor etc as you will do in the later subsection. 2. you can describe the overview based on fig 2 then and mention the input/output and novelties of each component, and readers will read it following the fig 2 and will be quite clear. 3. then in the following each subsection, you can in detail explain what each component is doing. 4. in the loss function section, you can name it as ``put everything together", and introduce the whole loss functions for the system -- remember to align the names of the loss functions with the ones in fig 2/3. }

%%%%%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%
%The underlying goal of portrait generation is to generate realistic portrait images which match a given input text description and an input photograph. In order to achieve this goal, the proposed Paint Robot leverages both fine-grained entity typing and inter-modal attention to explicitly characterize and model relationships between extracted text entities and image features. The methodology behind the proposed Paint Robot for portrait painting generation is described in detail below.
%The proposed Paint Robot text-and-photo-to-portrait synthesis 



==> backup/task.tex <==
\section{Task Definition}
As shown in Figure \ref{fig:TaskDef}, given an input photo and text description of the target portrait, the task is to generate a portrait with virtual features matching the content and style information inferred from the photo and text description, respectively. 

% \begin{figure}
% \centering
% \begin{tabular}{c}
% \includegraphics[width=8cm,height=8cm,keepaspectratio]{coling2020/img/task_definition4.pdf}
% \end{tabular}
% \caption{Input: photo and text description, output: generated portrait. \heng{do we also feed in unstructured text description? if so add that into the figure. Maybe we can drop this figure because figure 2 already includes task?}}
% %\heng{Attributes Selection -> Attribute Extraction; Paint Robot -> Portrait; maybe also show baseline results without text as input}}
% \label{fig:TaskDef}
% \end{figure}

%\heng{Xiaodan: can you start to put up a section about task definition, put in an example of input and output, with the input include all text descriptions, structured properties and extracted properties?}

% XXX check clustered results and give a walk through example



==> backup/textAttention.tex <==
\subsection{Attribute and Context Representations}
\label{sec:textAttn}

\heng{what do you mean by 'context' here?}

\heng{too vague, expand it and walk it through examples}
\heng{add Haoyang's advice on assigning different weights to different attribute types?}

we first compute an entity attribute context vector $c^e$ based on attention mechanism \cite{Bahdanau2015} \heng{what kind of attention is it? attention from what to what?} as:
\begin{equation}
\mathbf{c}^e = \sum_i a_i^e \mathbf{e}_i
\label{eq:c^e}
\end{equation}
\spencer{Need to clearly define $\mathbf{e}_i$ and $\mathbf{r}_j$.}
where the attention weights $a^e$ can be obtained as:
\begin{equation}
\mathbf{a}^e = \text{Softmax} (\mathbf{v}^e \tanh(\mathbf{W}^{e_1} \mathbf{s}+\mathbf{W}^{e_2} \mathbf{e}_i))
\label{eq:a^e}
\end{equation}
where $v^{e}$, $W^{e_1}$ and $W^{e_2}$ denote trainable parameters and bias terms are omitted for simplicity. Then a sentence context vector $c^r$ is computed as:
\begin{equation}
\mathbf{c}^r = \sum_j a_j^r \mathbf{r}_j
\label{eq:c^r}
\end{equation}
where the attention weights $a^r$ can be obtained as:
\begin{equation}
\mathbf{a}^r = \text{Softmax} (\mathbf{v}^r \tanh(\mathbf{W}^{r_1} \mathbf{s}+\mathbf{W}^{r_2} \mathbf{r}_j))
\label{eq:a^r}
\end{equation}
where $\mathbf{v}^{r}$, $\mathbf{W}^{r_1}$ and $\mathbf{W}^{r_2}$ are trainable parameters. Finally we input the concatenation of both the entity attribute context vector $\mathbf{c}^e$ and the sentence context vector $\mathbf{c}^r$, denoted as $\mathbf{c}$, as the text features.
\bo{emphasize the contribution of the joint representation for multinodality}



==> backup/texttoimage.tex <==

{\flushleft{\textbf{Text to Image:}}} 

\heng{maybe these methods are limited to certain tasks/scenarios? explain}
There have been many attempts at generating high-resolution images based on text descriptors~\cite{ReedAYLSL16,ZhangXLZHWM16,AttnGAN}. %Of the current state of the art methods for text-to-image synthesis, 
Generative Adversarial Networks (GANs) \cite{NIPSGAN} have become the predominant solution for this task. 
%Reed \etal 
\cite{ReedAYLSL16} first introduces a conditional DC-GAN architecture with matching-aware discriminator loss which 
%to enable image synthesis based on text descriptions. This method 
achieves positive results for generating low-resolution images ($64 \times 64$), but it is not equally successful in higher resolution generation.
% However, this method suffers from an undesirable separation between natural image distributions and generated image distributions in high dimensional spaces \cite{ArjovskyB17}. 
To address this problem, Zhang \etal \cite{ZhangXLZHWM16} proposes Stacked Generative Adversarial Networks (StackGAN) that first generates low resolution images and make refinements thereafter. \cite{zhang2018photographic} further proposes hierachically-nested losses that refines images in multiple steps. \cite{Lao2019DualAI} uses dual inference over conditional and unconditional latent variables for disentanglement of content and style. Rather than starting from low resolution image generation,  \cite{hong2018inferring} first constructs semantic layouts from text and generates images based on them. Despite promising results, the methods above incorporate only the global sentence features without considering the fine-grained entity information and thus yield unsatisfactory results when the input sentences are complex.


Xu \etal \cite{AttnGAN} proposes Attentional GAN (AttnGAN) to enable the generative networks to be trained on words of higher relevance. %In this method, a
An \textit{inter-modal} attention mechanism is developed to compute the similarity between the generated image and the relevant text description. \cite{qiao2019mirrorgan} considers both sentence- and word- level features in attention mechanism to improve the semantic consistency. \cite{tan2019semantics} also proposes a new semantic consistency module and an attention competition model to improve the semantic consistency of generated images. \heng{add comparison; point out why we need photo as part of input}





%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \heng{add these papers:
% % %[Scott Reed, et al, ICML, 2016]
% % %The images are generated by Yen-Hao Chen, Po-Chun Chien, Jun-Chen Xie, Tsung-Han Wu.
% % %Han Zhang, Tao Xu, Hongsheng Li, Shaoting Zhang, Xiaogang Wang, Xiaolei Huang, Dimitris Metaxas, “StackGAN: Text to Photo-realistic Image Synthesis with Stacked Generative Adversarial Networks”, ICCV, 2017
% % %https://arxiv.org/abs/1903.05854
% % % Shen et al., 2019
% % 
% }

%, which suffers from generating unsatisfying images for complex sentences with object interactions.

%On the other hand, 

%The highly challenging task of generating high-resolution images on the basis of text descriptors is a matter of great interest in the research community

% https://arxiv.org/abs/1902.10740

% %added by Yuqian
% Text-to-Image Synthesis Tasks Explored in Natural Images: mostly attributes extraction and object synthesis. Still very challenging in complicated scene generation. Not sure about painting generation.\\
% [Simple Objects like birds and flowers]\\

% 1. MirrorGAN: Learning Text-to-image Generation by Redescription, CVPR'19\\
% 2. Semantics-enhanced Adversarial Nets for Text-to-Image Synthesis, ICCV'19\\
% 3. Dual Adversarial Inference for Text-to-Image Synthesis, ICCV'19\\
% [Complicated Scenes]\\
% 4. Semantic Object Accuracy for Generative Text-to-Image Synthesis\\
% [Survey]\\
% 5. A Survey and Taxonomy of Adversarial Neural Networks for Text-to-Image Synthesis\\
% 6. Trends in Integration of Vision and Language Research: A Survey of Tasks, Datasets, and Methods
